Collaborative Insurance Sustainability and Network Structure

The peer-to-peer (P2P) economy has been growing with the advent of the Internet, with well known brands such as Uber or Airbnb being examples thereof. In the insurance sector the approach is still in its infancy, but some companies have started to explore P2P-based collaborative insurance products (eg. Lemonade in the U.S. or Inspeer in France). The actuarial literature only recently started to consider those risk sharing mechanisms, as in Denuit and Robert (2021) or Feng et al. (2021). In this paper, describe and analyse such a P2P product, with some reciprocal risk sharing contracts. Here, we consider the case where policyholders still have an insurance contract, but the first self-insurance layer, below the deductible, can be shared with friends. We study the impact of the shape of the network (through the distribution of degrees) on the risk reduction. We consider also some optimal setting of the reciprocal commitments, and discuss the introduction of contracts with friends of friends to mitigate some possible drawbacks of having people without enough connections to exchange risks.

==> lettre/tik1.tex <==


\tikzset{every picture/.style={line width=0.75pt}} %set default line width to 0.75pt        

\begin{tikzpicture}[x=0.75pt,y=0.75pt,yscale=-1,xscale=1]
%uncomment if require: \path (0,454); %set diagram left start at 0, and has height of 454

%Curve Lines [id:da11771822581058888] 
\draw    (57,136) .. controls (73.45,168.6) and (107.65,196.26) .. (166.02,170.32) ;
\draw [shift={(168.7,169.1)}, rotate = 154.98] [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.08]  [draw opacity=0] (8.93,-4.29) -- (0,0) -- (8.93,4.29) -- cycle    ;
%Curve Lines [id:da4499278601527311] 
\draw    (52.7,100.1) .. controls (69.23,57.63) and (103.02,5.16) .. (174.52,44.87) ;
\draw [shift={(176.7,46.1)}, rotate = 209.91] [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.08]  [draw opacity=0] (8.93,-4.29) -- (0,0) -- (8.93,4.29) -- cycle    ;
%Shape: Rectangle [id:dp6678374901753734] 
\draw   (9.7,102.1) -- (151.7,102.1) -- (151.7,135.1) -- (9.7,135.1) -- cycle ;
%Shape: Circle [id:dp08841717465673549] 
\draw  [fill={rgb, 255:red, 208; green, 2; blue, 27 }  ,fill opacity=1 ] (171,54.85) .. controls (171,46.1) and (178.1,39) .. (186.85,39) .. controls (195.6,39) and (202.7,46.1) .. (202.7,54.85) .. controls (202.7,63.6) and (195.6,70.7) .. (186.85,70.7) .. controls (178.1,70.7) and (171,63.6) .. (171,54.85) -- cycle ;
%Shape: Circle [id:dp11243822889178678] 
\draw  [fill={rgb, 255:red, 74; green, 144; blue, 226 }  ,fill opacity=1 ] (168.7,169.1) .. controls (168.7,160.35) and (175.8,153.25) .. (184.55,153.25) .. controls (193.3,153.25) and (200.4,160.35) .. (200.4,169.1) .. controls (200.4,177.85) and (193.3,184.95) .. (184.55,184.95) .. controls (175.8,184.95) and (168.7,177.85) .. (168.7,169.1) -- cycle ;
%Curve Lines [id:da9397629976720023] 
\draw    (197,68) .. controls (212.23,84.59) and (235.27,96.38) .. (263.1,88.85) ;
\draw [shift={(265.7,88.1)}, rotate = 162.76] [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.08]  [draw opacity=0] (8.93,-4.29) -- (0,0) -- (8.93,4.29) -- cycle    ;
%Curve Lines [id:da4636504177528814] 
\draw    (200.4,174.1) .. controls (215.63,190.69) and (238.67,202.48) .. (266.5,194.95) ;
\draw [shift={(269.1,194.2)}, rotate = 162.76] [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.08]  [draw opacity=0] (8.93,-4.29) -- (0,0) -- (8.93,4.29) -- cycle    ;
%Curve Lines [id:da6098564078474662] 
\draw    (200.7,44.85) .. controls (223.01,24.72) and (259.43,21.3) .. (284.42,40.27) ;
\draw [shift={(286.7,42.1)}, rotate = 220.03] [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.08]  [draw opacity=0] (8.93,-4.29) -- (0,0) -- (8.93,4.29) -- cycle    ;
%Curve Lines [id:da8980291876852439] 
\draw    (189.7,152.85) .. controls (212.01,132.72) and (248.43,129.3) .. (273.42,148.27) ;
\draw [shift={(275.7,150.1)}, rotate = 220.03] [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.08]  [draw opacity=0] (8.93,-4.29) -- (0,0) -- (8.93,4.29) -- cycle    ;

% Text Node
\draw (15,110) node [anchor=north west][inner sep=0.75pt]   [align=left] {insurance \& graphs};
% Text Node
\draw (57,198) node [anchor=north west][inner sep=0.75pt]  [color={rgb, 255:red, 74; green, 144; blue, 226 }  ,opacity=1 ] [align=left] {Charpentier \textit{et al.} (2021)};
% Text Node
\draw (118,7) node [anchor=north west][inner sep=0.75pt]  [color={rgb, 255:red, 208; green, 2; blue, 27 }  ,opacity=1 ] [align=left] {Feng \textit{et al.} (2021)};
% Text Node
\draw (293,31) node [anchor=north west][inner sep=0.75pt]  [color={rgb, 255:red, 208; green, 2; blue, 27 }  ,opacity=1 ] [align=left] {homogeneous network (complete)};
% Text Node
\draw (271,79) node [anchor=north west][inner sep=0.75pt]  [color={rgb, 255:red, 208; green, 2; blue, 27 }  ,opacity=1 ] [align=left] {heterogeneous risks };
% Text Node
\draw (281,140) node [anchor=north west][inner sep=0.75pt]  [color={rgb, 255:red, 74; green, 144; blue, 226 }  ,opacity=1 ] [align=left] {heterogeneous network (random graph)};
% Text Node
\draw (275,185) node [anchor=north west][inner sep=0.75pt]  [color={rgb, 255:red, 74; green, 144; blue, 226 }  ,opacity=1 ] [align=left] {homogeneous risk};


\end{tikzpicture}


==> lettre/tik2.tex <==


\tikzset{every picture/.style={line width=0.75pt}} %set default line width to 0.75pt        

\begin{tikzpicture}[x=0.75pt,y=0.75pt,yscale=-1,xscale=1]
%uncomment if require: \path (0,454); %set diagram left start at 0, and has height of 454

%Straight Lines [id:da13555364773040168] 
\draw    (471.85,173.85) -- (528.85,169.85) ;
%Straight Lines [id:da6094422139865602] 
\draw    (471.85,173.85) -- (492.85,129.85) ;
%Straight Lines [id:da9310855530464252] 
\draw    (474.85,58.85) -- (531.85,54.85) ;
%Straight Lines [id:da19349013135666226] 
\draw    (474.85,58.85) -- (501.85,68.85) ;
%Straight Lines [id:da768170639047624] 
\draw    (474.85,58.85) -- (495.85,14.85) ;
%Straight Lines [id:da8203570678995376] 
\draw    (474.85,58.85) -- (521.85,28.85) ;
%Straight Lines [id:da9961518899263033] 
\draw    (456.85,33.85) -- (474.85,58.85) ;
%Curve Lines [id:da4668582485170176] 
\draw    (57,136) .. controls (73.45,168.6) and (107.65,196.26) .. (166.02,170.32) ;
\draw [shift={(168.7,169.1)}, rotate = 154.98] [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.08]  [draw opacity=0] (8.93,-4.29) -- (0,0) -- (8.93,4.29) -- cycle    ;
%Curve Lines [id:da6432055637323363] 
\draw    (52.7,100.1) .. controls (69.23,57.63) and (103.02,5.16) .. (174.52,44.87) ;
\draw [shift={(176.7,46.1)}, rotate = 209.91] [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.08]  [draw opacity=0] (8.93,-4.29) -- (0,0) -- (8.93,4.29) -- cycle    ;
%Shape: Rectangle [id:dp2740168019568038] 
\draw   (9.7,102.1) -- (151.7,102.1) -- (151.7,135.1) -- (9.7,135.1) -- cycle ;
%Shape: Circle [id:dp9681686837207121] 
\draw  [fill={rgb, 255:red, 208; green, 2; blue, 27 }  ,fill opacity=1 ] (171,54.85) .. controls (171,46.1) and (178.1,39) .. (186.85,39) .. controls (195.6,39) and (202.7,46.1) .. (202.7,54.85) .. controls (202.7,63.6) and (195.6,70.7) .. (186.85,70.7) .. controls (178.1,70.7) and (171,63.6) .. (171,54.85) -- cycle ;
%Shape: Circle [id:dp08843862364667843] 
\draw  [fill={rgb, 255:red, 74; green, 144; blue, 226 }  ,fill opacity=1 ] (168.7,169.1) .. controls (168.7,160.35) and (175.8,153.25) .. (184.55,153.25) .. controls (193.3,153.25) and (200.4,160.35) .. (200.4,169.1) .. controls (200.4,177.85) and (193.3,184.95) .. (184.55,184.95) .. controls (175.8,184.95) and (168.7,177.85) .. (168.7,169.1) -- cycle ;
%Curve Lines [id:da5637954328553408] 
\draw    (197,68) .. controls (212.23,84.59) and (235.27,96.38) .. (263.1,88.85) ;
\draw [shift={(265.7,88.1)}, rotate = 162.76] [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.08]  [draw opacity=0] (8.93,-4.29) -- (0,0) -- (8.93,4.29) -- cycle    ;
%Curve Lines [id:da3956122194697549] 
\draw    (200.4,174.1) .. controls (215.63,190.69) and (238.67,202.48) .. (266.5,194.95) ;
\draw [shift={(269.1,194.2)}, rotate = 162.76] [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.08]  [draw opacity=0] (8.93,-4.29) -- (0,0) -- (8.93,4.29) -- cycle    ;
%Curve Lines [id:da7139354696032174] 
\draw    (200.7,44.85) .. controls (223.01,24.72) and (259.43,21.3) .. (284.42,40.27) ;
\draw [shift={(286.7,42.1)}, rotate = 220.03] [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.08]  [draw opacity=0] (8.93,-4.29) -- (0,0) -- (8.93,4.29) -- cycle    ;
%Curve Lines [id:da12834098578864173] 
\draw    (189.7,152.85) .. controls (212.01,132.72) and (248.43,129.3) .. (273.42,148.27) ;
\draw [shift={(275.7,150.1)}, rotate = 220.03] [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.08]  [draw opacity=0] (8.93,-4.29) -- (0,0) -- (8.93,4.29) -- cycle    ;
%Shape: Circle [id:dp38312066892434726] 
\draw  [fill={rgb, 255:red, 248; green, 231; blue, 28 }  ,fill opacity=1 ] (450,33.85) .. controls (450,30.07) and (453.07,27) .. (456.85,27) .. controls (460.63,27) and (463.7,30.07) .. (463.7,33.85) .. controls (463.7,37.63) and (460.63,40.7) .. (456.85,40.7) .. controls (453.07,40.7) and (450,37.63) .. (450,33.85) -- cycle ;
%Shape: Circle [id:dp035550349877065845] 
\draw  [fill={rgb, 255:red, 208; green, 2; blue, 27 }  ,fill opacity=1 ] (468,58.85) .. controls (468,55.07) and (471.07,52) .. (474.85,52) .. controls (478.63,52) and (481.7,55.07) .. (481.7,58.85) .. controls (481.7,62.63) and (478.63,65.7) .. (474.85,65.7) .. controls (471.07,65.7) and (468,62.63) .. (468,58.85) -- cycle ;
%Shape: Circle [id:dp7303159380918265] 
\draw  [fill={rgb, 255:red, 248; green, 231; blue, 28 }  ,fill opacity=1 ] (489,14.85) .. controls (489,11.07) and (492.07,8) .. (495.85,8) .. controls (499.63,8) and (502.7,11.07) .. (502.7,14.85) .. controls (502.7,18.63) and (499.63,21.7) .. (495.85,21.7) .. controls (492.07,21.7) and (489,18.63) .. (489,14.85) -- cycle ;
%Shape: Circle [id:dp7519688356502323] 
\draw  [fill={rgb, 255:red, 248; green, 231; blue, 28 }  ,fill opacity=1 ] (515,28.85) .. controls (515,25.07) and (518.07,22) .. (521.85,22) .. controls (525.63,22) and (528.7,25.07) .. (528.7,28.85) .. controls (528.7,32.63) and (525.63,35.7) .. (521.85,35.7) .. controls (518.07,35.7) and (515,32.63) .. (515,28.85) -- cycle ;
%Shape: Circle [id:dp3881412501759318] 
\draw  [fill={rgb, 255:red, 248; green, 231; blue, 28 }  ,fill opacity=1 ] (495,68.85) .. controls (495,65.07) and (498.07,62) .. (501.85,62) .. controls (505.63,62) and (508.7,65.07) .. (508.7,68.85) .. controls (508.7,72.63) and (505.63,75.7) .. (501.85,75.7) .. controls (498.07,75.7) and (495,72.63) .. (495,68.85) -- cycle ;
%Shape: Circle [id:dp4125742942515316] 
\draw  [fill={rgb, 255:red, 248; green, 231; blue, 28 }  ,fill opacity=1 ] (525,54.85) .. controls (525,51.07) and (528.07,48) .. (531.85,48) .. controls (535.63,48) and (538.7,51.07) .. (538.7,54.85) .. controls (538.7,58.63) and (535.63,61.7) .. (531.85,61.7) .. controls (528.07,61.7) and (525,58.63) .. (525,54.85) -- cycle ;
%Shape: Circle [id:dp9148623106591096] 
\draw  [fill={rgb, 255:red, 248; green, 231; blue, 28 }  ,fill opacity=1 ] (447,148.85) .. controls (447,145.07) and (450.07,142) .. (453.85,142) .. controls (457.63,142) and (460.7,145.07) .. (460.7,148.85) .. controls (460.7,152.63) and (457.63,155.7) .. (453.85,155.7) .. controls (450.07,155.7) and (447,152.63) .. (447,148.85) -- cycle ;
%Shape: Circle [id:dp3106318070459624] 
\draw  [fill={rgb, 255:red, 74; green, 144; blue, 226 }  ,fill opacity=1 ] (465,173.85) .. controls (465,170.07) and (468.07,167) .. (471.85,167) .. controls (475.63,167) and (478.7,170.07) .. (478.7,173.85) .. controls (478.7,177.63) and (475.63,180.7) .. (471.85,180.7) .. controls (468.07,180.7) and (465,177.63) .. (465,173.85) -- cycle ;
%Shape: Circle [id:dp13202832296480949] 
\draw  [fill={rgb, 255:red, 248; green, 231; blue, 28 }  ,fill opacity=1 ] (486,129.85) .. controls (486,126.07) and (489.07,123) .. (492.85,123) .. controls (496.63,123) and (499.7,126.07) .. (499.7,129.85) .. controls (499.7,133.63) and (496.63,136.7) .. (492.85,136.7) .. controls (489.07,136.7) and (486,133.63) .. (486,129.85) -- cycle ;
%Shape: Circle [id:dp1126059415101649] 
\draw  [fill={rgb, 255:red, 248; green, 231; blue, 28 }  ,fill opacity=1 ] (512,143.85) .. controls (512,140.07) and (515.07,137) .. (518.85,137) .. controls (522.63,137) and (525.7,140.07) .. (525.7,143.85) .. controls (525.7,147.63) and (522.63,150.7) .. (518.85,150.7) .. controls (515.07,150.7) and (512,147.63) .. (512,143.85) -- cycle ;
%Shape: Circle [id:dp8499506236852243] 
\draw  [fill={rgb, 255:red, 248; green, 231; blue, 28 }  ,fill opacity=1 ] (492,183.85) .. controls (492,180.07) and (495.07,177) .. (498.85,177) .. controls (502.63,177) and (505.7,180.07) .. (505.7,183.85) .. controls (505.7,187.63) and (502.63,190.7) .. (498.85,190.7) .. controls (495.07,190.7) and (492,187.63) .. (492,183.85) -- cycle ;
%Shape: Circle [id:dp3719839398604835] 
\draw  [fill={rgb, 255:red, 248; green, 231; blue, 28 }  ,fill opacity=1 ] (522,169.85) .. controls (522,166.07) and (525.07,163) .. (528.85,163) .. controls (532.63,163) and (535.7,166.07) .. (535.7,169.85) .. controls (535.7,173.63) and (532.63,176.7) .. (528.85,176.7) .. controls (525.07,176.7) and (522,173.63) .. (522,169.85) -- cycle ;

% Text Node
\draw (15,110) node [anchor=north west][inner sep=0.75pt]   [align=left] {insurance \& graphs};
% Text Node
\draw (57,198) node [anchor=north west][inner sep=0.75pt]  [color={rgb, 255:red, 74; green, 144; blue, 226 }  ,opacity=1 ] [align=left] {Charpentier \textit{et al.} (2021)};
% Text Node
\draw (118,7) node [anchor=north west][inner sep=0.75pt]  [color={rgb, 255:red, 208; green, 2; blue, 27 }  ,opacity=1 ] [align=left] {Feng \textit{et al.} (2021)};
% Text Node
\draw (292,34.4) node [anchor=north west][inner sep=0.75pt]    {$d( i) =n-1,\ \forall i$};
% Text Node
\draw (183,45.4) node [anchor=north west][inner sep=0.75pt]  [color={rgb, 255:red, 255; green, 255; blue, 255 }  ,opacity=1 ]  {$i$};
% Text Node
\draw (181,160.4) node [anchor=north west][inner sep=0.75pt]  [color={rgb, 255:red, 255; green, 255; blue, 255 }  ,opacity=1 ]  {$i$};
% Text Node
\draw (288,142.4) node [anchor=north west][inner sep=0.75pt]    {$d( i) \sim \ D$};
% Text Node
\draw (291,13) node [anchor=north west][inner sep=0.75pt]   [align=left] {number of connections};
% Text Node
\draw (285,122) node [anchor=north west][inner sep=0.75pt]   [align=left] {number of connections};
% Text Node
\draw (269,78.4) node [anchor=north west][inner sep=0.75pt]    {$X( i) =\ell \left( p_{i} ,\underbrace{p_{1} ,...,p_{i-1} ,p_{i+1} ,...,p_{n}}\right)$};
% Text Node
\draw (272,186.4) node [anchor=north west][inner sep=0.75pt]    {$X( i) =\ell \left( p_{i} ,\underbrace{p_{i_{1}} ,...,p_{i_{d( i)}}}\right)$};


\end{tikzpicture}


==> name.tex <==
Changement Climatique et Assurance

Par 	Arthur Charpentier, Professeur UQAM & Université de Rennes 1
	

Impact du changement climatique
Munich Re (2014) a montré, au regard des données des 50 dernières années que la fréquence des catastrophes météorologiques et climatiques ne cesse d’augmenter dans le monde. Et les pertes assurées également, en grande partie à cause du développement de l’assurance. Selon Mills (2009), 16 % des pertes liées aux conditions météorologiques étaient assurées dans les années 1980, pour atteindre 37,6 % en moyenne au cours des dix dernières années. La croissance économique, l’augmentation des richesses, l’industrialisation de zones vulnérables et la concentration des populations expliquent une grande partie de l’augmentation, comme le note Botzen et al. (2010).
  
Figure 1 : catastrophes météorologiques et climatiques dans le monde, modifié de Munich Re (2014).
 
World Weather-Related Natural Catastrophes By Overall And Insured Losses, 1980-2018 

 
Figure 2 : Montants des sinistres causés par les catastrophes météorologiques et climatiques dans le monde, modifié de Munich Re (2014).
Les liens entre cette augmentation de la fréquence et de la gravité de ces catastrophes (allant des vagues de chaleur aux épisodes froids, des sécheresses aux pluies diluviennes, ou encore aux tempêtes et ouragans) et le changement climatique sont encore mal connus. Comme le note IPCC (2013), de faibles changements sur la distribution moyenne des températures peuvent avoir de gros impacts sur les quantiles élevés. Vecchi & Knutson (2011) propose par exemple une étude passionnante sur la prévision des phénomènes cycloniques tropicaux en Amérique du Nord. Mais comme le souligne Changnon et al. (2000), la hausse exponentielle des coûts est très largement expliquée par des facteurs sociaux. Et ces catastrophes posent de réels défis aux assureurs de par leur caractère largement imprévisible.
Au cours des 20 dernières années, le coût global des aléas naturels en France s’élève  à 34 milliards d’euros, et ce pour les seuls assureurs.  Selon un chiffrage décrit dans FFSA (2009), la charge totale pour les 20 prochaines années pourrait être le double (en euros constants), la moitié de cette charge étant expliquée par des facteurs liés aux évolutions soco-économiques (augmentation de la somme assurée en grande partie, mais aussi migration vers des zones à risque), et la moitié étant expliquée par des facteurs liés au changement climatique.
Mais au-delà de ces catastrophes, le changement climatique impacte tous les secteurs de l’assurance.L’augmentation des précipitations en Europe (non seulement en moyenne, mais aussi avec une hausse des crues éclair) va affecter les infrastructures souterraines, ou situées à proximité des cours d’eau. Les propriétés situées sur les côtes sont menacées par l’élévation du niveau des mers. Les risques liés aux inondations constituent une catégorie de catastrophe très impactée par le changement climatique : selon la CCR, les plus fortes évolutions attendues des sinistres catastrophes des 30 prochaines années seront relatives à la submersion marine (+60 %) et aux inondations par débordement et ruissellement (+20 %). Un autre risque est celui lié aux sécheresses, qui endommage aussi les bâtiments par affaissement des sols. La canicule de l’été 2003 en France a causé une hausse des réclamations en assurance construction de l’ordre de 20 %. En assurance vie, la canicule de 2003, exceptionnelle par sa durée, a là aussi montré l’impact potentiel du changement climatique sur les personnes les plus vulnérables (enfants très jeunes, personnes âgées, et malades chroniques). L’assurance agricole est également impactée par les sécheresses et les inondations. Les sécheresses augmentent aussi le risque d’incendie, pouvant détruire forêts et récoltes. En assurance automobile, les conditions climatiques restent une explication à bon nombre de sinistres. Le nombre d’accidents augmente fortement lors des journées (très) chaudes. La grêle est l’événement climatique qui cause le plus de dommages directs en assurance automobile.
L’assurabilité des risques climatiques
Godard (1997), reprenant des idées développées par Ewald (1986) a montré que le développement de la société industrielle s’était traduit par une augmentation de la demande de protection. Cette protection peut être offerte par des Etats, mais aussi par des compagnies d’assurance, si le risque le permet. Plusieurs critères sont nécessaires pour que le risque soit « assurable ».
Légalement, un contrat d’assurance ne peut être valide que si l’occurrence des sinistres satisfait un caractère aléatoire. En France, l’article 1 de la loi du 13 Juillet 1982 relative à l’indemnisation des biens assurés suite à une catastrophe naturelle mentionne que « sont considérés comme les effets des catastrophes naturelles, au sens de la présente loi, les dommages matériels directs ayant eu pour cause déterminante l’intensité anormale d’un agent naturel [...] ». Est-il anormal d’avoir des inondations récurrentes dans des zones potentiellement inondables comme par exemple l’ancien lit d’une rivière ? D’un point de vue actuariel, la perte maximale ne doit pas être trop importante. Les tempêtes de 1999 (non couvertes par le mécanisme dit Cat Nat) ont ainsi causé des dommages supérieurs à la « perte maximale possible » calculée par le secteur de l’assurance. Ces risques doivent aussi être mutualisables. Pour que le mécanisme d’assurance fonctionne, comme le rappelle Ewald (1986), « le risque est collectif [...] ce n’est en effet que sur l’étendue d’une population qu’un risque devient calculable. Le travail d’un assureur est précisément de constituer cette population par sélection et diversification des risques. L’assurance [...] passe par la socialisation des risques ». Quand un même évènement engendre 3 millions de demandes d’indemnisation (comme les tempêtes survenues en décembre 1999 en France), on peut difficilement parler de mutualisation des risques, « the contribution of the many to the misfortune of the few » (pour reprendre la devise du Lloyd’s). Mais plus important, il faut qu’un marché de l’assurance existe, avec des assureurs prêts à offrir une couverture, et des assurés prêts à souscrire de tels contrats.
Les solutions d’assurance en Europe
Les assureurs se sont efforcés d’offrir une couverture dans la mesure du possible. Ces solutions font souvent intervenir les compagnies d’assurance. Il n’y a généralement pas d’intervention de l’Etat, et les couvertures pour ces risques sont facultatives.  Dans ce cas, le taux de pénétration  dépend de la perception du risque par les citoyens. Dans d’autres pays, au contraire, les assureurs n’interviennent pas, et c’est l’Etat qui prend à sa charge les sinistres (à partir du budget ou d’un fonds spécifique alimenté par une taxe sur les contrats d’assurance). Dans le cas de la France, il existe un mécanisme mixte dit Cat Nat, basé sur un mélange d’assurance obligatoire et d’intervention publique. Enfin, la couverture doit être proposée par les assureurs, mais la souscription de tels contrats est facultative. La Figure 3 tente de résumer le patchwork européen.
 
Figure 3 : couverture d’assurance des catastrophes naturelles en Europe, modifié de Mills (2009).
Ce subtil équilibre entre assureurs privés et Etat évolue dans le temps. Car tous ont peur des conséquences financières des catastrophes. L’Etat qui avait offert sa caution – par exemple en tant qu’ « assureur en dernier ressort » – se voit contraint de faire figurer cet engagement dans son budget. Et les assureurs savent que le changement climatique va se traduire par des exigences en terme de capital, comme le montre la Figure 4.
 
Figure 4 : impact du changement climatique sur le capital réglementaire, modifié de ABI (2005).
L’articulation entre le marché de l’assurance et l’Etat peut se voir comme un effet de subvention du marché de l’assurance, pour couvrir les risques climatiques, comme le note Stern (2006).
Le rôle des assureurs
Le changement climatique engendre davantage d’incertitude pour les assureurs, et il n’est alors pas surprenant de les voir s’impliquer pour tenter de proposer des solutions. On peut ainsi souligner les actions collaboratives sur Climate Wise Group, qui tente d’encourager la prévention. L’exemple des inondations survenues en 2007 au Royaume Uni est intéressant à ce titre. Comme le note ABI (2007), l’évaluation et la gestion du risque d’inondation ont montré de nombreuses faiblesses. Mills (2009) rapporte que l’industrie de l’assurance britannique s’est alors engagée dans le financement de travaux de recherche sur les inondations en milieu urbain. Les assureurs britanniques (mais le même phénomène a été observé en France) ont alors cherché à être impliqués dans les processus d’aménagement du territoire, de planification d’utilisation des terres, et la conception et la mise en œuvre des codes de construction.
Plusieurs travaux soulignent que les gains engendrés par les mesures de précaution sont souvent colossaux par rapport à leur coût. En 2004, la Banque Mondiale avait ainsi calculé que pour toutes les catastrophes naturelles survenues dans les années 1990, 40 milliards d’€ investis dans des mesures de prévention auraient permis de réduire le coût total de 280 milliards d’€. On retrouve le même ordre de grandeur lorsque ABI (2007) déclare que chaque livre sterling dépensée dans des mesures de prévention permettrait d’économiser 6 livres sterling en coûts de réparation, lors d’inondations. Un groupe de travail sur l’économie de l’adaptation, impulsé en particulier par Swiss Re et McKinsey, a vu le jour ces dernières années avec pour but de systématiser ce type d’analyse en vue d’optimiser les choix d’investissement d’adaptation (ECA 2010). Par exemple, une des multiples études de cas issue de ces travaux, portant sur la côte du Golfe du Mexique aux Etats-Unis, montre qu’investir 50 milliards de $ dans les vingt prochaines années, principalement dans le remblayage des plages et les modifications du code de construction (voir figure), permettrait une réduction de 135 milliards de $ dans le coût des catastrophes futures .  
Finalement on peut saluer l’apparition dans les dernières années du concept de « pertes et dommages » dans les négociations internationales ayant lieu dans le cadre de la convention cadre de l’ONU sur le changement climatique. Ce concept a abouti à la création lors de la COP19 de 2013,  du « mécanisme international de Varsovie pour les pertes et dommages» (UNFCCC 2013) repris lors de la COP21 de 2015, dont le fonctionnement reste encore largement à préciser mais vise à incorporer plusieurs aspects: (i) réduction et transfert des risques liés aux catastrophes climatiques, (ii) adaptation au changement climatique, (iii) considérations politiques telles que le dédommagement des pays les plus vulnérables par les pays développés, principaux responsables du problème (Surminski and Lopez 2014). Le rôle des assureurs dans ce dispositif international devra être précisé mais il est clair que son existence fournit d’emblée un cadre adapté permettant aux assureurs d’aborder l’ensemble des questions présentées ci-dessus en lien avec les multiples secteurs concernés (par exemple par le biais d’entités telles que Munich climate insurance initiative). Parmi les multiples points restant à préciser, il sera nécessaire de pouvoir statuer sur la nature anthropogénique ou non des catastrophes climatiques couvertes par le dispositif, afin de déterminer en conséquence le bien-fondé et le montant des indemnités. Pour cette raison, cette question de l’attribution causale des événements climatiques fait actuellement l’objet de nombreuses recherches en sciences du climat (James et al. 2014).

ABI (2005). Financial risks of climate change. Technical report, Association of British Insurers.
ABI (2007). Summer floods 2007 : Learning the lessons. Technical report, Association of British Insurers.
Botzen, W. J. W., van den Bergh, J. C. J. M., and Bouwer, L. M. (2010). Climate change and increased risk for the insurance sector: a global perspective and an assessment for the netherlands. Natural Hazards, 52(3), 577–598.
Ewald, F. (1986). L’Etat providence. Grasset
FFSA (2009). Synthèse de l’étude relative à l’impact du changement climatique et de l’aménagement du territoire sur la survenance d’événements naturels en France. FFSATechnical report.
IPCC (2013). Climate Change 2013 : The Physical Science Basis. Contribution of Working Group I to the Fifth Assessment Report of the Intergovernmental Panel on Climate Change. Cambridge University Press.
Mills (2009).  From Risk to Opportunity: Insurer Responses to Climate Change http://www.climate-insurance.org/upload/pdf/Mills2008_risk-to-opportunity.pdf
Munich Re (2014). Loss events worldwide 1980 - 2013., Geo risks research. Munich Reinsurance Group. http://www.munichre.com/en/reinsurance/business/non-life/natcatservice/index.html.
Stern, N. (2006). Stern review : the economics of climate change. Cambridge University Press.
Vecchi, G. A. & Knutson, T. R. (2011). Estimating annual numbers of Atlantic hurricanes missing from the hurdat database (1878–1965) using ship track density. Journal of Climate, 24(6), 1736–1746.
MCII. (2012). Munich climate insurance initiative. http://www.climate-insurance.org/ 
UNFCCC. (2013). Decision 2/CP.19 Warsaw international mechanism for loss and damage associated with climate change impacts. Retrieved February 10, 2014, from http://unfccc. int/resource/docs/2013/cop19/eng/10a01.pdf
Surminski S., A. Lopez (2014): Concept of loss and damage of climate change – a new challenge for climate decision-making? A climate science perspective. Climate and Development
James R., Otto F., Parker H., Boyd E., Cornforth R., Mitchell D., Allen M. (2014) Characterizing loss and damage from climate change. Nat Clim Change 4:938–939



==> tikz/tikzit_setup.tex <==
% Tickszit
\usepackage[svgnames]{xcolor}
\usetikzlibrary{decorations.markings}
\usetikzlibrary{positioning, shapes.geometric}
\pagestyle{empty}


\pgfdeclarelayer{edgelayer}
\pgfdeclarelayer{nodelayer}
\pgfsetlayers{edgelayer,nodelayer,main}


% Node styles
\tikzstyle{orange_node}=[fill={rgb,255: red,255; green,128; blue,0}, draw=black, shape=circle, minimum size=6mm]

\tikzstyle{green node}=[fill={rgb,255: red,42; green,211; blue,4}, draw=black, shape=circle, minimum size=6mm]

\tikzstyle{red node}=[fill=red, draw=black, shape=circle, minimum size=6mm]
\tikzstyle{blue node}=[fill={rgb,255: red,73; green,185; blue,255}, draw=black, shape=circle, minimum size=6mm]

% Edge styles
\tikzstyle{black edge}=[-, fill=none]
\tikzstyle{arrow head left}=[fill=none, <-]
